ALTO: Alternating Latent Topologies for Implicit 3D Reconstruction

This work introduces alternating latent topologies (ALTO) for high-fidelity reconstruction of implicit 3D surfaces from noisy point clouds. Previous work identifies that the spatial arrangement of latent encodings is important to recover detail. One school of thought is to encode a latent vector for each point (point latents). Another school of thought is to project point latents into a grid (grid latents) which could be a voxel grid or triplane grid. Each school of thought has tradeoffs. Grid latents are coarse and lose high-frequency detail. In contrast, point latents preserve detail. However, point latents are more difficult to decode into a surface, and quality and runtime suffer. In this paper, we propose ALTO to sequentially alternate between geometric representations, before converging to an easy-to-decode latent. We find that this preserves spatial expressiveness and makes decoding lightweight. We validate ALTO on implicit 3D recovery and observe not only a performance improvement over the state-of-the-art, but a runtime improvement of 3-10$\times$. Project website at https://visual.ee.ucla.edu/alto.htm/.

==> point-grid-alternating-cvpr2023 (Copy) (1)/sec_abstract.tex <==
\begin{abstract}
This work introduces alternating latent topologies (ALTO) for high-fidelity reconstruction of implicit 3D surfaces from noisy point clouds. Previous work identifies that the spatial arrangement of latent encodings is important to recover detail. One school of thought is to encode a latent vector for each point (point latents). Another school of thought is to project point latents into a grid (grid latents) which could be a voxel grid or triplane grid. Each school of thought has tradeoffs. Grid latents are coarse and lose high-frequency detail. In contrast, point latents preserve detail. However, point latents are more difficult to decode into a surface, and quality and runtime suffer. In this paper, we propose ALTO to sequentially alternate between geometric representations, before converging to an easy-to-decode latent. We find that this preserves spatial expressiveness and makes decoding lightweight. We validate ALTO on implicit 3D recovery and observe not only a performance improvement over the state-of-the-art, but a  runtime improvement of 3-10$\times$. Project website at \url{https://visual.ee.ucla.edu/alto.htm/}.
\end{abstract}

==> point-grid-alternating-cvpr2023 (Copy) (1)/sec_conclusions.tex <==
\section{Discussion and Conclusion}


In summary, this paper has adopted a different philosophy from the SOTA in surface detail recovery. We rely neither on point latents~\cite{boulch2022poco} or grid latents~\cite{peng2020convolutional} alone, but alternate between topologies. The output of ALTO is a spatially expressive latent that is also topologically easy-to-decode into a 3D surface. This breaks a Pareto tradeoff that previous works have posited between spatial expressiveness and decoding complexity. For this reason, it is not surprising that our method reconstructs more detailed 3D surfaces with faster runtimes than state-of-the-art (\cref{fig:teaser} and~\cref{tab:runtime}).

% \begin{table}[t]
%     \label{tab:ubfc}
%     % \vskip 0.05in
%   \begin{center}
%   \resizebox{\linewidth}{!}{
%   \begin{tabular}{lccccccc} 
%     \toprule
  
%     Method & $\#$ Parameters & Memory (GB) &  Inference time (s) \\
%     \midrule
%     ConvONet ($3 \times 128^2$) & 7,812,705 & 1.80 & 0.97\\
%     ConvONet ($64 ^3$)  & 4,166,657 & 2.06 & 1.11 \\ 
%     POCO~\cite{boulch2022poco} & 12,790,454 & 5.55  & 62.41 \\
%     \midrule
%     Ours ($3 \times 128^2$) & 2,713,889 & 1.74 & 4.86\\
%     Ours  ($64 ^3$) & 4,778,433 & 2.70 &4.48 \\
%     Ours (w/ our decoder, $3 \times 128^2$) & 2,763,073 & 3.00  & 6.93\\
%     Ours (w/ our decoder, $64 ^3$) & 5,064,801& 3.20 & 6.98\\
%     \bottomrule
%   \end{tabular}}
%  \end{center}
%   \caption{Our method is faster than POCO. Time reported includes mesh generation.}
% \end{table}


The idea of alternating latent topologies could have implications beyond surface reconstruction. Concurrent research has introduced unusual latent topologies, known as \textbf{irregular latents} that show compelling performance benefits for neural fields~\cite{zhang20223dilg}. One can imagine alternating not only between point, triplane, and voxel latents, but also throwing irregular latents in the mix. We are also curious to see if alternating topologies can improve performance on a wide range of tasks in neural fields that require spatially expressive latents, such as semantic or affordance fields.

\section{Acknowledgement}
This project was supported by the US DoD LUCI (Laboratory University Collaboration Initiative) fellowship and partially supported by ARL grants W911NF-20-2-0158 and W911NF-21-2-0104 under the cooperative A2I2 program. D.P. is supported by the Swiss National Science Foundation under grant number P500PT\_206946. G.W. is supported by Samsung, Stanford HAI, and a PECASE from the ARO. L.G. is also supported by an ONR Vannevar Bush Faculty Fellowship. A.K. is also supported by a DARPA Young Faculty Award, NSF CAREER Award, and Army Young Investigator Award.  
%\jj{Finally, discuss how conditional implicit fields generation methods are useful. For example, in "Variational GIGA" or "Synergies Between Affordance and Geometry" they use it for grasping affordance predictions. "Neural Descriptor Fields" models descriptor fields using implicit fields. Some classic applications of conditional implicit fields generation are "PiFu" and 'DiSN'.}


% Our model can reduce the quantization effect due to the grid discretization in the grid form by introducing iterative alternation between grid and point forms. Since point form enables feature learning at individual point level, it is thus capable of encoding more fine-grained local features for conditional occupancy field generation.


==> point-grid-alternating-cvpr2023 (Copy) (1)/sec_intro.tex <==
\section{Introduction}
\label{sec:intro}


% our method is general. can be applied to existing grid or point-based methods. 
% can be simply plugged in for other neural fields
% tri-plane-based: efficient but lacks communication between the UNets. 

Reconstructing surfaces from noisy point clouds is an active problem in 3D computer vision. Today, conditional neural fields offer a promising way to learn surfaces from noisy point clouds. Alternatives like voxel regression or mesh estimation are limited by cubic complexity and the requirement of a mesh template, respectively. Recent work has successfully used conditional neural fields to reconstruct 3D surfaces as an occupancy function. A conditional neural field takes as input a query coordinate and conditions this on a latent representation, e.g., feature grids. % of a noisy point cloud. 
The spatial expressiveness of the latent representation impacts the overall surface reconstruction quality. 

\begin{figure*}[t]
  \centering
%   \fbox{\rule{0pt}{3in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=\linewidth]{figures/network_architecture/network_architecture}

   \caption{\textbf{An overview of our method.} Given input surface points, we obtain an implicit occupancy field with iterative alternation between features in the forms of points and 2D or 3D grids (\cref{sec:alternating}). Then we decode the occupancy values for query points with a learned attention-based interpolation from neighboring grids (\cref{sec:attention}).}
   \label{fig:pipeline}
\end{figure*}

To achieve spatial expression, a neural field is conditioned on a latent space of features (\textbf{latents}) from the conditional input. In 3D surface reconstruction the input point cloud is transformed into latents arranged in some topological structure. \textbf{Point latents} occur when each point in the input point cloud is assigned a latent vector~\cite{boulch2022poco}. \textbf{Triplane latents} are formed when point latents are projected into a 3-axis grid~\cite{lionar2021dynamic, peng2020convolutional}. The triplane latent is not as spatially expressive as freeform points, but the lower spatial complexity makes it easier to decode. \textbf{Voxel latents} are another type of grid latent where latents are arranged in a feature volume~\cite{peng2020convolutional, tang2021sa}. 
% A voxel latent is considered in-between the point and triplane in its spatial expressivity and ease of decoding. \achuta{zhen can you address gordon's comment and add 1-2 refs here?}

To reconstruct detailed surfaces, recent state-of-the-art methods try to preserve point latents as long as possible. Because point latents are spatially expressive, methods based on point latents are considered state-of-the-art for detailed surface reconstruction~\cite{boulch2022poco,erler2020points2surf}. However, using point latents in this way has some tradeoffs. It is difficult to correlate a query with the unstructured topology of a point-based latent space, placing a burden on the decoder. Results from POCO~\cite{boulch2022poco} are shown in~\cref{fig:teaser} where runtime and high-quality detail like thin lampposts remain out of reach.

In this paper, we seek to blend the upside of different latent topologies, while minimizing downside. We present an alternating latent topology (ALTO) method. In contrast to previous work, our method does not stay with either point~\cite{boulch2022poco} or grid latents~\cite{peng2020convolutional}, but instead alternates back and forth between point and grid latents before converging to a final grid for ease-of-decoding. 

% ALTO can convert grid features back into point features after convolutional operations on grids, so point features with aggregated neighborhood information are learned at finer granularity with just a simple per-point multi-layer perceptron (MLP). For 2D grids, the MLP also provides an extra benefit of promoting communication among three planar features. We then project point features back to grid features for convolution. The alternation makes these two forms of features complementary: fine-grained per-point feature learning lead to better grid features and convolutional grid features can efficiently propagate both global and local features for each point. 
Our method is general. We can plug-in the ALTO component to existing grid-based conditional models \cite{peng2020convolutional,Chibane2020CVPR} to boost detail recovery. While we have shown that our method can generate occupancy fields, we expect gain of high-fidelity details for other neural fields, such as semantic or affordance fields \cite{vora2021nesf, jiang2021synergies}, where similar conditional techniques can be adopted.

We summarize our \textbf{contributions} as follows:
\begin{itemize}\itemsep=0cm
    \item{We introduce an iterative technique to blend the strengths of different latent topologies for high-fidelity conditional neural fields generation.}
    \item{We propose an attention-based decoder that replaces naive linear interpolation of feature-grids or computationally expensive point-wise attention while keeping compute burden in check.}


    % \item {We improve runtime over existing occupancy decoders via an attention-based mechanism that replaces linear interpolation of feature-grids and computationally expensive point-wise attentions.}
    
            \item {We demonstrate performance and runtime improvements over the highest-quality previous method~\cite{boulch2022poco}, as well as performance improvements over all other baselines.}
    % \item {Performance and runtime improvements over the highest-quality previous method~\cite{boulch2022poco}. Performance improvements over all other baselines.}
\end{itemize}





% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{3.5in} \rule{\linewidth}{0pt}}
%   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%   \caption{Maybe a teaser figure: our method is both fast and accurate compared with e.g. POCO and/or SA-ConvONet.}
%   \label{fig:teaser}
% \end{figure}





    % \item We propose a simple point-grid alternating block that converts point cloud features iteratively between two previous commonly \emph{yet} separately used forms: per-point form and grid (either 2D or 3D) form;
    
    % \item We incorporate this block into a hourglass framework and the resulting point-grid alternating U-Net architecture enables more efficient alternation between the two form; and 
    % \item Extensive empirical results on both object and scene-level synthetic and real-world datasets demonstrate that our method can learn better implicit representation for surface reconstruction.
    % \item (TBD) A new dataset which extract occupancy labels from 3D front dataset.
    % \item (TBD) A new occupancy decoder using attention mechanism based on our learned feature forms.



==> point-grid-alternating-cvpr2023 (Copy) (1)/sec_method.tex <==
\section{Method}

\label{sec:method}
There are three insights that motivate our approach: (1) conditioning on the right topology of the latent space is important; (2) previous neural fields for surface reconstruction condition on point or grid latents; (3) both point and grid latents have complementary strengths and weaknesses. Point latents are more spatially expressive but grid latents are easier to decode into a surface.

It might seem like a simple concatenation of point and grid latents would be sufficient. The problem is that point latents remain difficult to decode (even if concatenated with a grid latent). Therefore, our insight is to alternate between grid and point latents, and converge to a grid latent. For feature triplane latents, the alternation also permits communication between the individual planes, which in previous, grid-based works would have been fed into independent hourglass U-Nets~\cite{peng2020convolutional}. 

In this section, we introduce a version of ALTO as a point-grid alternating U-Net. An overview of the method is shown in~\cref{fig:pipeline}. We demonstrate how the convolutional grid form is learned in~\cref{sec:feature_grid}, our point-grid alternating network in~\cref{sec:alternating}, our attention-based decoder in~\cref{sec:attention} and training and inference in more detail in~\cref{sec:training}. 
 
\subsection{Convolutional Feature Grids}
\label{sec:feature_grid}

The input to our method is a noisy un-oriented point cloud $\mathcal{P}=\left\{\boldsymbol{p}_{i} \in \mathbb{R}^{3}\right\}_{i=1}^{S}$, where $S$ is the number of input points. We first use a shallow Point-Net~\cite{qi2017pointnet} to obtain the initial point features as in ConvONet~\cite{peng2020convolutional}. 
 These point features are then projected into three 2D grids (feature triplanes) $\{\mathbf{\Pi}_{xy}, \mathbf{\Pi}_{xz}, \mathbf{\Pi}_{yz}\} \in  \mathbb{R}^{H \times W \times d}$ or 3D grids (feature volumes) $\mathbf{V} \in  \mathbb{R}^{H \times W \times D \times d}$ before feeding into a 2D or 3D convolutional hourglass (U-Net) networks~\cite{cciccek20163d, ronneberger2015u}. $d$ is the number of feature channels. For feature volumes, we set $H = W = D = 64$ due to memory overhead of 3D-CNN and for feature triplanes, $H$ and $W$ can be set as high as 128 depending on the task.
 
% Seen from the lens of ConvONet~\cite{peng2020convolutional}, a key distinction is that we do not proceed with the grid latent, but instead iteratively alternate between grid and point latents to learn a fine-grained implicit representation for decoding occupancy.

\subsection{ALTO Latent to Blend Grid and Point Latents}
\label{sec:alternating}
Without loss of generality, we demonstrate ALTO in the context of blending grid and point latents. Note that 
naive concatenation of latents would not work, as the point latents are difficult to decode. The goal is to use ALTO to blend point latent characteristics into a grid latent via alternation. The alternating block is illustrated in~\cref{fig:alternation} and incorporated into a U-Net architecture. At each alternation, we first do grid-to-point conversion where convolutional grid features are transformed into point features, followed by point-to-grid conversion where extracted point features are transformed back into grid features for next alternation. 


\textbf{Grid-to-Point Conversion:} At each alternation, to aggregate local neighborhood information, we use convolutional operations for the grid features. We then project each point $p$ orthographically onto the canonical planes and query the feature values through bilinear interpolation for 2D grid and trilinear interpolation for 3D grid. For triplane latents, we sum together the interpolated features from each individual plane. 


\textbf{Point-to-Grid Conversion:} At each alternation, given the interpolated point features, we then process point features with an MLP in order to model individual point feature with finer granularity. For feature triplanes grid form, an MLP also gives an additional benefit of having individual plane features communicate with each other. The MLP is implemented with two linear
layers and one ReLU nonlinearity.
Projected point features falling within the same pixel or voxel cell will be aggregated using average pooling. If using triplane latents with each plane discretized at $H \times W$, this results in planar features with dimensionality $H \times W \times d$ 
or if using voxel latents we obtain dimensionality $H \times W \times D \times d$, where $d$ is the number of features.

We also adopt skip connections for both point features and grid features between two consecutive ALTO blocks, as illustrated in ~\cref{fig:alto_consecutive}.
The alternation needs to be implemented carefully to minimize runtime. Naively, we can alternate between triplanes or voxel latents using a U-Net and point latents using MLP, but that would require multiple network passes. Instead, we incorporate the point-grid alternating \emph{inside} each block of a U-Net, i.e. replacing original convolution-only block with ALTO block. We call this single U-Net, the ALTO U-Net. This also enables point and grid features blended at multiple scales and the number of alternation blocks depends on the number of levels of U-Net.


\subsection{Decoding ALTO latents using Attention}
\label{sec:attention}



As discussed in the previous section, ALTO provides a way to get a single latent that blends characteristics of different topologies. The advantage is that the final latent that ALTO converges to (hereafter, ALTO latent) can take on the topology that is easier to decode. 

For example, in the case of using ALTO to blend point and grid characteristics, we would like ALTO to converge to a final output in the simpler grid topology. Then, given the ALTO latent in grid form and any query point $\mathbf{q} \in \mathbb{R}^3$ in 3D space, our goal is to decode the learned feature and estimate the occupancy probability of each query point. ALTO benefits from attention on the decoder side. The ALTO latent is in grid form, but has spatial expressivity coming from the blended-in point latents. Standard grid latent decoding, e.g., bi-/tri-linear interpolation used in previous work~\cite{peng2020convolutional, lionar2021dynamic} would not preserve this spatial expressivity. 

\begin{figure}[t]
  \centering
%   \fbox{\rule{0pt}{3in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=\linewidth]{figures/attention/attention_4}
   \caption{\textbf{Attention-based decoder on neighboring grids (2D or 3D).} To obtain features of each query point for decoding occupancy value, we use learned interpolation from neighboring grids that improves occupancy prediction, while being more efficient than expansive point-wise attention mechanism (e.g. POCO~\cite{boulch2022poco}).}
   \label{fig:attention}
\end{figure}

To decode an ALTO latent, we propose an efficient attention-based mechanism
to replace the previous approach of linear interpolation on feature grids. While attention is not new, we leverage \emph{grid latent attention} to avoid heavy runtime issues of \emph{point latent attention}~\cite{boulch2022poco} that applies attention over a point-wise 3D neighborhood. As illustrated in \cref{fig:attention}, 
% besides the traditional linear interpolation, 
we consider the nearest grids (indices denoted as $\mathcal{N}(\mathbf{q})$), where $|\mathcal{N}|=9$ for triplane representation and $|\mathcal{N}|=27$ for volume representation, we call these areas as per-point neighbor feature patches $\mathbf{C}_{\{i \in \mathcal{N}\}}$. We define the query $Q$, key $K$, and value $V$ for our attention as follows:
\begin{equation}
\begin{aligned}
Q &= \text{MLP}(\mathbf{\psi(q)}),\\
K &= \text{MLP}(\mathbf{C}_{\{i \in \mathcal{N}(\mathbf{q})
\}}),\\
V &= \text{MLP}(\mathbf{C}_{\{i \in \mathcal{N}(\mathbf{q})
\}}),
\end{aligned}
\end{equation}
where $\mathbf{\psi(q)}$ is the linear interpolated feature value of the query points. Additionally, we  compute the displacement vector $\mathbf{d} \in \mathbb{R}^2$ or $\mathbb{R}^3$ which represents the spatial relationship between the projected query point coordinate and the nearest feature grid points. We use the subtraction relation~\cite{zhao2021point} in our attention scoring function:

\begin{equation}
A = \text{softmax}(\text{MLP}((Q-K)+\gamma(\mathbf{d}))),
\end{equation}
where $\gamma(\mathbf{d})$ works as a learnable positional encoding. In our implementation, $\gamma$ is an MLP with two fully-connected layers and activated by ReLU. We compute the attention-based interpolated per-point feature $F$ as:
\begin{equation}
F = A \odot (V + \gamma(\mathbf{d})).
\end{equation}
Note that the same positional encoding from above is added to $V$ and $\odot$ denotes the element-wise product operation. For the case of triplane representation, we use a single-head attention to extract the feature $F$ from each individual plane. The per-triplane features are then concatenated and used for the occupancy prediction.
For the case of the volume representation, we use multi-head attention for $h$ independently learned subspaces of $Q$, $K$, and $V$, where $h$ is a hyperparameter varying based on the experiment. Additional details are provided in the supplementary.
\begin{table*}[t]
    % \vskip 0.05in
  \begin{center}
  \resizebox{\linewidth}{!}{
  \begin{tabular}{lcccccccccccc} 
    \toprule
       \multirow{1}{*}{} & \multicolumn{4}{c}{\centering input points 3K} & \multicolumn{4}{c}{\centering input points 1K} & \multicolumn{4}{c}{\centering input points 300} \\
    \cmidrule(l){2-5} \cmidrule(l){6-9} \cmidrule(l){10-13} 
    Method & IoU $\uparrow$ & Chamfer-$L_1 \downarrow$ & NC$\uparrow$ & F-score$\uparrow$ & IoU $\uparrow$ & Chamfer-$L_1 \downarrow$ & NC$\uparrow$ & F-score$\uparrow$ & IoU $\uparrow$ & Chamfer-$L_1 \downarrow$ & NC$\uparrow$ & F-score$\uparrow$  \\
    \midrule
    ONet~\cite{mescheder2019occupancy} & 0.761 & 0.87 & 0.891 & 0.785 & 0.772 & 0.81 & 0.894 &  0.801 & 0.778 & 0.80 & 0.895 &0.806 \\
%   SPSR~\cite{kazhdan2013screened} &  \\
%   SPSR trimmed~\cite{kazhdan2013screened} &  \\
  ConvONet~\cite{peng2020convolutional} &0.884 & 0.44 & 0.938 & 0.942 & 0.859 & 0.50 & 0.929 & 0.918 &0.821 &0.59 & 0.907 & 0.883\\
%   DP-ConvONet~\cite{lionar2021dynamic} & 0.895 & 0.42 & 0.941 & 0.952 & \\
  POCO~\cite{boulch2022poco} & 0.926 & \textbf{0.30} & 0.950 & \textbf{0.984} & 0.884 & 0.40 & 0.928 & 0.950 & 0.808 & 0.61 & 0.892 & 0.869 \\
  \midrule
  ALTO (Encoder Only) &  \textbf{0.931} & \textbf{0.30} & 0.950 & 0.981 & 0.889 & 0.39 & 0.932 & 0.951 & 0.842 & 0.52 & 0.908 & 0.903\\
  ALTO &  0.930 & \textbf{0.30} & \textbf{0.952} & 0.980 & \textbf{0.905} & \textbf{0.35} & \textbf{0.940} &  \textbf{0.964} & \textbf{0.863} & \textbf{0.47} & \textbf{0.922} & \textbf{0.924} \\
    \bottomrule
  \end{tabular}}
 \end{center}\vspace{-5mm}
  \caption{\textbf{Performance on ShapeNet with various point density levels.} Input noisy point cloud with 3K, 1K and 300 input points from left to right. ALTO is our proposed method and ALTO (Encoder only) is an ablation that uses only our encoder with a non-attention based decoder.}
  \label{tab:shapenet}
\end{table*}

\begin{figure}
     \includegraphics[width=\linewidth]{figures/F_ablation.pdf}
      \hfill\subcaptionbox{GT}[0.22\linewidth]
    \hfill\subcaptionbox{Grid Latent~\cite{peng2020convolutional}}[0.28\linewidth]
    \hfill\subcaptionbox{~\cref{sec:alternating}\\\centering ``ALTO (Enc.)''}[0.24\linewidth]
    \hfill\subcaptionbox{~\cref{sec:alternating}+\ref{sec:attention}\\\centering ``ALTO''\label{fig:ablationd}}[0.27\linewidth]
    
    \caption{\textbf{Ablation analysis on ShapeNet.} Note the top inset showing the poles in the chair back (yellow). ALTO (Enc.) is ALTO (Encoder Only) and uses the latent space encoding proposed in~\cref{sec:alternating} with a standard decoder. The full ALTO method includes also the attention-based decoder in~\cref{sec:attention}.}
    \label{fig:ablation}
\end{figure}
Finally, we predict the occupancy of $\mathbf{q}$ using a small fully-connected occupancy network:
\begin{equation}
f_{\theta}(F) \rightarrow [0,1].
\end{equation}
The network $f_{\theta}$ consists of several ResNet blocks as in~\cite{peng2020convolutional}. The major difference to the original occupancy decoder in~\cite{peng2020convolutional} is that we do not bring in the absolute 3D coordinate of $\mathbf{q}$ as input since it theoretically breaks the translational equivalence property.

This concludes our description of our latent space encoding and attention decoding. In~\cref{fig:ablation} observe that the architectures we have proposed progressively improve detail from a standard grid formulation.



\subsection{Training and Inference}
\label{sec:training}

At training time, we uniformly sample query points $\mathcal{Q}$ and minimize the binary cross-entropy loss between the predicted occupancy value and ground-truth occupancy values written as: 
\begin{equation}
\mathcal{L}\left(\hat{o}_{\mathbf{q}}, o_{\mathbf{q}}\right) \! = \! \!- \!\!\sum_{\mathbf{q}\in \mathcal{Q}}\left[o_{\mathbf{q}} \log \left(\hat{o}_{\mathbf{q}}\right)\!+\!\left(1\!-\!o_{\mathbf{q}}\right) \log \left(1\!-\!\hat{o}_{\mathbf{q}}\right)\right]
\end{equation}
Our model is implemented in PyTorch~\cite{paszke2019pytorch} and uses the Adam optimizer~\cite{kingma2014adam} with a learning rate of $10^{-4}$. During inference, we use a form of Marching Cubes~\cite{lorensen1987marching} to obtain the mesh.

==> point-grid-alternating-cvpr2023 (Copy) (1)/sec_related.tex <==
\section{Related Work}
\label{sec:related}

%Representations for 3D scenes fall under three broad categories: explicit data structures, neural fields and conditional neural fields. Our work is most closely related to conditional neural fields, Section~\ref{ss:conditional}.
In this section, we discuss the most relevant literature on learning-based 3D reconstruction methods.
Based on their output, existing learning-based approaches can be categorized
as implicit or explicit-based representations. In this work, we primarily focus on implicit-based
representations as they are closely related to our method.

%\subsection{Explicit Data Structures}
\subsection{Explicit Representations}
\label{ss:explicit}

A common     shape representation is 2.5D depth maps, which can be inferred using 2D CNNs \cite{Kar2017NIPS, Hartmann2017ICCV, Paschalidou2018CVPR, Huang2018CVPR, Yao2018ECCV, Donne2019CVPR, Yao2019CVPR, Yu2020CVPR}.
However, 2.5D depth maps cannot capture the full 3D geometry. In contrast, voxels \cite{Maturana2015IROS, Wu2015NIPS, Brock2016ARXIV, Choy2016ECCV, Wu2016NIPS, Gadelha2017THREEDV, Rezende2016NIPS, Stutz2018CVPR, Xie2019ICCV, dai2020sg} naturally capture 3D object geometry,
by discretizing the shape into a regular grid. As voxel-based methods exhibit cubic space complexity that results
in high memory and computation requirements, several works tried to circumvent this with efficient space partitioning techniques \cite{Maturana2015IROS, Riegler2017CVPR, Tatarchenko2017ICCV, Haene2017ARXIV, Riegler2017THREEDV}.
Although these methods allow for increasing the voxel resolution and hence capturing more complex geometries,
their application is still limited. Recently, a promising new direction explored learning grid deformations
to better capture geometric details~\cite{Gao2020NIPS}. An alternative representation relies on pointclouds.
Point-based approaches \cite{Fan2017CVPR, Qi2017NIPS, Achlioptas2018ICML, Jiang2018ECCV, Thomas2019ICCV, Yang2019ICCV}
discretize the 3D space using points and are more light-weight and memory efficient. However, as they lack surface connectivity,
they require additional post-processing steps (\eg using Poisson Surface Reconstruction\cite{Kazhdan2006PSR})
for generating the final mesh. Instead, mesh-based methods~\cite{Liao2018CVPR, Groueix2018CVPR, Kanazawa2018ECCV, Wang2018ECCV, Yang2019ICCV, Gkioxari2019ICCV, Pan2019ICCV, Chen2019NIPS, Deng2020CVPR}
naturally yield smooth surfaces but they typically
require a template mesh~\cite{Wang2018ECCV}, which makes scaling them to arbitrarily complex
topologies difficult. Other works, proposed to also represent the geometry as an atlas of 
mappings~\cite{Groueix2018CVPR, Deng2020THREEDV, Ma2021CVPR}, which can result in
non-watertight meshes. To address limitations with learning explicit representations, 
implicit models~\cite{mescheder2019occupancy, Chen2019CVPR, Park2019CVPR,sitzmann2019siren } emerged as an alternative
more compact representation that yield 3D geometries at infinitely high resolutions using iso-surfacing operations
(\ie marching cubes). In this work, we capture 3D geometries implicitly,
using an occupancy field~\cite{mescheder2019occupancy}, as it faithfully can
capture complex topologies.

%Explicit data structures include point clouds, grids, voxels, and meshes. A \textbf{point cloud} organizes the geometric location of points into an array and are considered light-weight and efficient~\cite{qi2017pointnet,qi2017pointnet++}. In addition, point features can be processed at very fine granularity (i.e. at individual point level). However, point clouds cannot model topological relations. A \textbf{grid} is formed by projecting points into 2D or 3D planes, enabling conventional convolution kernels to learn local features~\cite{hua2018pointwise,xu2018spidercnn,atzmon2018point}. However, grids do not model the full volume, whereby one might appeal to a \textbf{voxel } data structure~\cite{choy20163d, maturana2015voxnet, dai2020sg, wu2016learning, wu20153d, xie2019pix2vox}. Unfortunately, voxel-based methods exhibit cubic space complexity, which limits performance. Alternatively, one can learn a \textbf{mesh}, consisting of vertices and faces~\cite{Liao2018CVPR,
%Groueix2018CVPR, Kanazawa2018ECCV, Wang2018ECCV, Yang2019ICCV, Pan2019ICCV}. Unfortunately, this typically requires a template mesh and arbitrary topologies are difficult to represent with a template mesh.  

\subsection{Neural Implicit Representations} 
\label{ss:implicit}

Unlike explicit representations that discretize the output space using voxels,
points or mesh vertices, implicit representations represent the 3D shape and appearance implicitly,
in the latent vectors of a neural network that learns a mapping between
a query point and a context vector to either a signed distance value
\cite{Park2019CVPR, Michalkiewicz2019ICCV, Atzmon2020CVPR, Gropp2020ICML,
Takikawa2021CVPR} or a binary occupancy value \cite{mescheder2019occupancy, Chen2019CVPR, Sitzmann2019NIPS}.
However, while these methods typically rely on a single global latent code, they cannot capture local details and
struggle scaling to more complicated geometries.
To address this, several works \cite{Saito2019ICCV, Xu2019NIPS, Saito2020CVPR} explored 
pixel-aligned implicit representations, that rely on both global and local image features
computed along a viewing direction. While, these approaches are able to capture fine-grained geometric details,
they rely on features that are computed from images, hence are limited to image-based inputs
with known camera poses.

Our work falls in the category of methods that perform 3D reconstructions from points. Among the first
to explore this direction were \cite{peng2020convolutional, Chibane2020CVPR,
Jiang2020CVPR}. To increase the expressivity of the underlying representation and to be able to capture
complex geometries, instead of conditioning on a global latent code, these works condition on local per-point
features. For example, Jiang \etal ~\cite{Jiang2020CVPR} leverage shape priors by conditioning on a 
patch-based representation of the point cloud. Other works \cite{peng2020convolutional,lionar2021dynamic,tang2021sa}, 
utilize grid-based convolutional features extracted from feature planes \cite{lionar2021dynamic},
feature volumes \cite{Chibane2020CVPR, tang2021sa} or both
\cite{peng2020convolutional}. An alternative line of work,
\cite{williams2022neural} introduce a test-time optimization mechanism to refine the per-point features predicted on a
feature volume. Concurrently, POCO~\cite{boulch2022poco}, propose to estimate per-point features, which are then
refined based on the per-point features of their neighboring points using an attention-based mechanism. A similar idea is also explored in Points2Surf~\cite{Erler2020ECCV} that introduces
a patch-based mechanism to decide the sign of the implicit function.  Our work is closely related to
POCO~\cite{boulch2022poco} that can faithfully capture higher-frequency details due its point-wise latent coding.
However, the lack of a grid-like structure places extra complexity on the attention-based aggregation module, 
which results in a higher computation cost. AIR-Net~\cite{giebenhain2021air} applied local attention to reduce the computation but limits its operating range to objects.
% and problems with generalizability, especially in areas with fine detail.
In this work, we propose conditioning on a hybrid representation of points and grid latents.
%It is reminescent of work from in 3D semantic segmentation that fuses points and voxels~\cite{liu2019point}.
In particular, instead of fusing points and grids, we demonstrate that it is the point and grid \emph{alternation}
between points and grids that enables recovery of more detail than POCO~\cite{boulch2022poco},
while reducing compute time by an order of magnitude.

\subsection{Obtaining Implicit Fields from Images} 
\label{ss:implicit}

As the previous methods require 3D supervision, several recent works
propose combining implicit representations with surface 
\cite{Niemeyer2020CVPR, Yariv2020NIPS} or volumetric \cite{Mildenhall2020ECCV}
rendering techniques in order to learn 3D object geometry and texture from
images. Among the most extensively used implicit representations are Neural
Radiance Fields (NeRF) \cite{Mildenhall2020ECCV} that combine an implicit representation
with volumetric rendering to perform a novel view synthesis. In particular, they employ
a neural network that maps a 3D point along a viewing direction to a color and a density value.
NeRFs are trained using only posed images. On the other hand \cite{Niemeyer2020CVPR, Yariv2020ARXIV}
combined occupancy fields~\cite{mescheder2019occupancy} and signed distance functions (SDFs) with
surface rendering in order to recover the geometry and appearance of 3D objects. 

Though we only demonstrate a case study in occupancy field in this paper, our proposed method is general and can be readily plugged into all kinds of other neural fields for better 3D point feature encoding. We leave that as future exploration.

%\subsection{Unconditional Neural Fields}
%\label{ss:unconditional}

%The term \textbf{neural field} is used to describe a practice of encoding the occupancy function into the weights of a neural network. For the scope of this paper, a \textbf{query} is an input 3D coordinate for which we seek to predict its binary occupancy. An \textbf{unconditional neural field} takes as input a coordinate query and outputs occupancy (or similar surface representation). The input query coordinate is not conditioned on another input to the neural field. Many of the early methods in neural fields were unconditional, such as Neural Radiance Fields (NeRF)~\cite{}, Scene Representation Networks (SRNs)~\cite{Sitzmann2019NIPS}, and Deep Signed Distance Functions (DeepSDFs)~\cite{park2019deepsdf}, PiGAN~\cite{Chan2021CVPR}, EG3D~\cite{Chan2021eg3d}. These methods took the computer vision community by storm for their ability to recover complex topology at virtually infinite resolution (as the query coordinate is a continuous variable). Unfortunately, the weights of the network are \emph{ad-hoc} to the scene that one seeks to query an input point on. Without conditioning on another input, unconditional neural fields are limited to applications where one is able to re-train models for each new, 3D scene. 

%\subsection{Conditional Neural Fields} 
%\label{ss:conditional}

%A \textbf{conditional neural field} conditions the query coordinate with another input: a representation of the 3D scene to be queried. Unfortunately, the 3D representation is difficult to decode into occupancy maps. For example, some conditional neural fields have represented the conditional 3D input with a global latent vector~\cite{mescheder2019occupancy}. Even with coordinate-based activation functions~\cite{Sitzmann2019NIPS}, a global latent vector is not \textbf{spatially expressive}, i.e., where spatial features of the input point cloud are preserved in the representation. Therefore, recovered occupancy maps from such methods are blurry.

%In an attempt to preserve detail in surface reconstruction, recent work has shown that improving the spatial expressiveness of the conditional point cloud features is important. LIG~\cite{Jiang2020CVPR} conditions on a patch-based representation of the point cloud, IF-Net~\cite{Chibane2020CVPR} and NDF~\cite{Chibane2020ARXIV} condition on multi-scale pyramids, ConvONet~\cite{Peng2020ECCV}, DP-ConvONet~\cite{lionar2021dynamic}, and Sign-Agnostic ConvONet~\cite{tang2021sa} condition on grid-based convolutional features. While these methods have more spatial expressiveness than latent codes, the use of patches or grids provides coarser spatial expressiveness than a point representation. To further increase spatial expressiveness, the current state of the art is POCO~\cite{boulch2022poco} and  NKF~\cite{williams2022neural} which condition on point-based latent codes. \jj{instead of relying on no code argument, we combine NKF and "Local Implicit Grid Representations for 3D Scenes" as  a test-time optimization methods. These methods require either solving for some equation or optimizing for latent codes during the test-time, so might not be suitable for time-critical applications, or with mobile computes.} \achuta{JJ would you mind writing your comment in directly?}The code for NKF is not yet released, so it is difficult to use it as a comparison point, and we will consider POCO as the closest state-of-the-art to benchmark against. As compared to grid-based approaches, POCO shows an ability to recover higher-frequency detail, thanks to the point-wise latent coding. However, the lack of a grid-like structure places complexity on the attention-based decoder to blend neighboring point features. This leads to a high compute cost and problems with generalizability, especially in areas with fine detail. 

%In contrast to previous work, this paper conditions on a hybrid representation of points and grids. It is reminescent of work from in 3D semantic segementation that fuses points and voxels~\cite{liu2019point}. However, rather than fusing points and voxels, this paper shows that it is point and grid \emph{alternation} between points and grids that enables recovery of even more detail than POCO~\cite{boulch2022poco}, while reducing compute time by an order of magnitude. %It should also be mentioned that the point-grid alternating U-Net can be readily plugged into various existing methods such as~\cite{boulch2022poco,williams2022neural} to generate better point features from our implicit representation that can benefit decoding occupancy.

% \jj{3DILG: a concurrent work with irregular latents. needs auto-regressive generation of points. slow}
% \jj{AIR-Nets: I don't know too much about this work...}



\begin{figure*}[t]
%   \centering
%   \fbox{\rule{0pt}{3in} \rule{0.9\linewidth}{0pt}}
  \includegraphics[width=\linewidth]{figures/unet_grid/unet_grid_final.pdf} 
  \hfill\subcaptionbox{}[0.45\linewidth]
  \hfill\subcaptionbox{\label{fig:alto_consecutive}}[0.48\linewidth]
  
  \vspace{-.2cm}\caption{\textbf{An illustration of our ALTO encoder.} (a) As an example, we show the ALTO block instantiated by alternating between two latent topologies: point and triplanes via an ``in-network'' fashion, i.e. within each level of an hourglass framework U-Net.  `Concatenate' refers to concatenation of the ALTO block output triplane in the downsampling stage and the ALTO block input triplane in the corresponding upsampling stage. (b) We expand on ALTO block to illustrate the sequential grid-to-point and point-to-grid conversion. There are skip connections for both point and grid features between two consecutive levels in the ALTO U-Net. }
  \label{fig:alternation}
\end{figure*}
%  \zw{still need to iterate with Despi on a few changes of this fig.} \achuta{Rather than using Point-Grid we may want to do ALTO(Point, TriPlane) so it's written in a functional form?}.


%\begin{figure*}[t]
%  \centering
%   \fbox{\rule{0pt}{3in} \rule{0.9\linewidth}{0pt}}
%   \includegraphics[width=\linewidth]{figures/unet.JPG}

%   \caption{An overarching illustration of the general idea: point-grid alternating U-Net}
%   \label{fig:alternation}
%\end{figure*}
%\begin{figure*}[t]
%  \centering
%   \fbox{\rule{0pt}{3in} \rule{0.9\linewidth}{0pt}}
%   \includegraphics[width=\linewidth]{figures/unet_grid/unet_grid_2}
%
%   \caption{An overarching illustration of the general idea: point-grid alternating U-Net}
%   \label{fig:alternation}
%\end{figure*}

%Learning Continuous Environment Fields via Implicit Functions

==> point-grid-alternating-cvpr2023 (Copy) (1)/sec_results.tex <==
\section{Experimental Evaluation}
\label{sec:results}

% \achuta{Please put placeholders figures in (with captions) while you are waiting on the SN generalization results.}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}
%     \begin{subfigure}[t]{\columnwidth}
%     \centering
%     \vspace{-1.2em}
%     \begin{subfigure}[b]{0.20\linewidth}
% 		\centering
%         Input
%     \end{subfigure}%
%     \hfill%
%     \begin{subfigure}[b]{0.20\linewidth}
% 		\centering
%         OccNet
%     \end{subfigure}%
%     \hfill%
%     \begin{subfigure}[b]{0.20\linewidth}
% 		\centering
%         CvxNet-5
%     \end{subfigure}%
%     \hfill%
%     \begin{subfigure}[b]{0.20\linewidth}
% 		\centering
%         CvxNet-25
%     \end{subfigure}%
%     \hfill%
%     \begin{subfigure}[b]{0.20\linewidth}
%         \centering
%         Ours
%     \end{subfigure}
%     \vspace{-2.2em}
%     \vskip\baselineskip%
%     \begin{subfigure}[b]{0.20\linewidth}
% 		\centering
% 		\includegraphics[width=\linewidth]{gfx/shapenet/cars/input_886246c286351bc6cc010a80df5d3c87}
%     \end{subfigure}%
%     \hfill%
%     \begin{subfigure}[b]{0.20\linewidth}
% 		\centering
% 		\includegraphics[width=\linewidth]{gfx/shapenet/cars/occnet_886246c286351bc6cc010a80df5d3c87}
%     \end{subfigure}%
%     \hfill%
%     \begin{subfigure}[b]{0.20\linewidth}
% 		\centering
% 		\includegraphics[width=\linewidth]{gfx/shapenet/cars/cvxnet_5_886246c286351bc6cc010a80df5d3c87}
%     \end{subfigure}%
%     \hfill%
%     \begin{subfigure}[b]{0.20\linewidth}
% 		\centering
% 		\includegraphics[width=\linewidth]{gfx/shapenet/cars/cvxnet_25_886246c286351bc6cc010a80df5d3c87}
%     \end{subfigure}%
%     \hfill%
%     \begin{subfigure}[b]{0.20\linewidth}
% 		\centering
% 		\includegraphics[width=\linewidth]{gfx/shapenet/cars/ours_886246c286351bc6cc010a80df5d3c87}
%     \end{subfigure}%
%     \vspace{-2.2em}
%     \vskip\baselineskip%
%     \begin{subfigure}[b]{0.20\linewidth}
%     	\centering
% 		\includegraphics[trim=30 30 30 30,clip,width=\textwidth]{gfx/shapenet/airplanes/input_1b3c6b2fbcf834cf62b600da24e0965}
%     \end{subfigure}%
%     \hfill%
%     \begin{subfigure}[b]{0.20\linewidth}
%     	\centering
% 		\includegraphics[width=0.8\linewidth]{gfx/shapenet/airplanes/occnet_1b3c6b2fbcf834cf62b600da24e0965}
%     \end{subfigure}%
%     \hfill%
%     \begin{subfigure}[b]{0.20\linewidth}
%     	\centering
% 		\includegraphics[width=0.8\linewidth]{gfx/shapenet/airplanes/cvxnet_5_1b3c6b2fbcf834cf62b600da24e0965}
%     \end{subfigure}%
%     \hfill%
%     \begin{subfigure}[b]{0.20\linewidth}
%     	\centering
% 		\includegraphics[width=0.8\linewidth]{gfx/shapenet/airplanes/cvxnet_25_1b3c6b2fbcf834cf62b600da24e0965}
%     \end{subfigure}%
%     \hfill%
%     \begin{subfigure}[b]{0.20\linewidth}
%     	\centering
% 		\includegraphics[width=0.8\linewidth]{gfx/shapenet/airplanes/ours_1b3c6b2fbcf834cf62b600da24e0965}
%     \end{subfigure}%
%     \vspace{-1.2em}
%     \vskip\baselineskip%
%     \begin{subfigure}[b]{0.20\linewidth}
%     	\centering
% 		\includegraphics[width=0.8\textwidth]{gfx/shapenet/chairs/input_1c199ef7e43188887215a1e3ffbff428}
%     \end{subfigure}%
%     \hfill%
%     \begin{subfigure}[b]{0.20\linewidth}
%     	\centering
% 		\includegraphics[width=0.8\textwidth]{gfx/shapenet/chairs/occnet_1c199ef7e43188887215a1e3ffbff428}
%     \end{subfigure}%
%     \hfill%
%     \begin{subfigure}[b]{0.20\linewidth}
%     	\centering
% 		\includegraphics[width=0.8\textwidth]{gfx/shapenet/chairs/cvxnet_5_1c199ef7e43188887215a1e3ffbff428}
%     \end{subfigure}%
%     \hfill%
%     \begin{subfigure}[b]{0.20\linewidth}
%     	\centering
% 		\includegraphics[width=0.8\textwidth]{gfx/shapenet/chairs/cvxnet_25_1c199ef7e43188887215a1e3ffbff428}
%     \end{subfigure}%
%     \hfill%
%     \begin{subfigure}[b]{0.20\linewidth}
%     	\centering
% 		\includegraphics[width=0.8\textwidth]{gfx/shapenet/chairs/ours_1c199ef7e43188887215a1e3ffbff428}
%     \end{subfigure}%
%     \end{subfigure}\\[1.2em]
%     \begin{subfigure}[t]{0.95\columnwidth}
%         \resizebox{\columnwidth}{!}{%
%         \centering
%         \begin{tabular}{l||c|ccc}
%             \toprule
%             IoU & OccNet & CvxNet - 5 & CvxNet - 25 & Ours \\
%             \midrule
%             cars & 0.763 & 0.650 & 0.666 &  \bf{0.697} \\
%             planes & 0.451 & 0.425 & 0.448 &  \bf{0.454} \\
%             chairs & 0.432 & 0.364 & 0.392 &  \bf{0.412} \\
%             \bottomrule
%         \end{tabular}}
%     \end{subfigure}
%     \caption{{\bf Single Image 3D Reconstruction on ShapeNet}. We compare
%     Neural Parts to OccNet and CvxNet with $5$ and $25$ primitives. Our model
%     yields semantic and more accurate reconstructions with $5\times$ less
%     primitives.}
%     \label{fig:shapenet_results}
%     \vspace{-1.2em}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% We demonstrate the performance of our method compared with state-of-the-art methods on single object reconstruction~(\cref{sec:object}), scene-level reconstruction~(\cref{sec:scene}) and synthetic-to-real generalization on real-world scans~(\cref{sec:real}). 


\subsection{Datasets, Metrics, and Baselines}
\textbf{Object Level Datasets:} For evaluation on object-level reconstruction, we use ShapeNet~\cite{chang2015shapenet}.
% , ABC~\cite{koch2019abc}, Famous\cite{erler2020points2surf} and Things10k~\cite{erler2020points2surf}.
In particular, ShapeNet~\cite{chang2015shapenet} contains watertight meshes of object shapes in 13 classes. For fair comparison, we use the same train/val splits and 8500 objects for testing as described in~\cite{boulch2022poco,peng2020convolutional}. Points are obtained by randomly sampling 
% 3000 points 
from each mesh and adding Gaussian noise with zero mean and standard deviation of 0.05. 
% For ABC, Famous and Things10k, we follow a similar protocol, as discussed in the supplement.


\textbf{Scene-Level Datasets:} For scene level evaluation, we use Synthetic Rooms dataset~\cite{peng2020convolutional} and ScanNet-v2~\cite{Dai2017CVPR}. In total, we use 5000 synthetic room scenes with walls, floors and ShapeNet objects randomly placed together. We use an identical train/val/test split as prepared in prior work~\cite{peng2020convolutional,boulch2022poco}, and Gaussian noise with zero mean and 0.05 standard deviation. ScanNet-v2 contains 1513 scans from real-world scenes that cover a wide range of room types. Since the provided meshes in ScanNet-v2 are not watertight, models are trained on the Synthetic Rooms dataset and tested on ScanNet-v2, which also enables some assessment of Sim2Real performance of various methods.

\textbf{Evaluation Metrics:} The quantitative evaluation metrics used in data tables are standard metrics that enable us to form comparisons to prior work. These include: volumetric IoU, Chamfer-$L_{1}$ distance $\times 10^2$, and normal consistency (NC). A detailed definition of each metric can be found in the Occupancy Networks paper~\cite{mescheder2019occupancy}. We also include an F-Score metric~\cite{tatarchenko2019single} with threshold value $1\%$. 

\textbf{Baselines for Comparison:} As noted by Boulch et al.~\cite{boulch2022poco}, baseline methods often perform better in the settings of the original papers. In the same spirit, we thus strictly adapt the protocol of the state-of-the-art (SOTA) paper POCO~\cite{boulch2022poco} for evaluation protocol. In addition to POCO, other baselines we include are  SPSR~\cite{kazhdan2013screened}, ONet~\cite{mescheder2019occupancy} and ConvONet~\cite{peng2020convolutional}.
% , and Points2Surf~\cite{erler2020points2surf}. 
Note that we omit NFK~\cite{williams2022neural} from our evaluations, as they have not made their code publicly available.

\textbf{Our Method:} ``Our method'' is ALTO. ALTO combines~\cref{sec:alternating}~+~\cref{sec:attention}, and is shown in~\cref{fig:ablationd}. Figures/tables use ALTO to denote the proposed method. If we are considering an ablation analysis we will use ALTO with parentheses, e.g., ``ALTO (Encoder Only)'', and the table caption will specify the ablation. To demonstrate ALTO with different latent topologies , for object-level reconstruction, we use alternation between point and feature triplanes and the resolution of initial individual plane $H = W = 64$. For scene-level reconstruction, we use alternation between point and feature volumes and the resolution $H = W = D = 64$. 



\begin{figure}[t]
%   \fbox{\rule{0pt}{3in} \rule{\linewidth}{0pt}}
 \includegraphics[width=\linewidth]{figures/F_shapenet2.pdf}\vspace{-2mm}
       \hfill\subcaptionbox{GT}[0.20\linewidth]
    \hfill\subcaptionbox{Input (1K)}[0.21\linewidth]
    \hfill\subcaptionbox{CONet~\cite{peng2020convolutional}}[0.21\linewidth]
    \hfill\subcaptionbox{POCO~\cite{boulch2022poco}}[0.20\linewidth]
       \hfill\subcaptionbox{\textbf{ALTO}}[0.14\linewidth]
      
     \vspace{-.2cm}\caption{\textbf{Object-level comparisons on ShapeNet.} On the car, ALTO recovers the detail of having both side mirrors.}
  \label{fig:shapenet}
\end{figure}

% \begin{table*}[t]
% \small
% \centering
% \resizebox{\linewidth}{!}{
%   \begin{tabular}{lccccccccccccc}
%     \toprule
%     \multirow{1}{*}{} & \multicolumn{3}{c}{\centering ABC} & \multicolumn{5}{c}{\centering Famous} & \multicolumn{5}{c}{\centering Things10k} \\
%     \cmidrule(l){2-4} \cmidrule(l){5-9}  \cmidrule(l){10-14} 
%     Method & no-n. & var-n. & max-n. & no-n. & med-n.& max-n.& sparse &dense & no-n. & med-n.& max-n.& sparse &dense \\
%     \midrule
%     DeepSDF~\cite{park2019deepsdf} & 8.41 & 12.51 & 11.34 & 10.08 & 9.89 & 13.17 & 10.41 & 9.49 & 9.16 & 8.83 & 12.28 & 9.56 & 8.35 \\
%     AtlasNet~\cite{groueix2018papier} & 4.69 & 4.04 & 4.47 & 4.69 & 4.54 & 4.14 & 4.91 & 4.35 & 5.29 & 5.19 & 4.90 & 5.64 & 5.02\\
%     SPSR~\cite{kazhdan2013screened} & 2.49 & 3.29 & 3.89 & 1.67 & 1.80 & 3.41 & 2.17 & 1.60 & 1.78 & 1.81 & 3.23 & 2.35 & 1.57\\
%     Points2Surf~\cite{erler2020points2surf} & 1.80& 2.14 & 2.76 & 1.41 & 1.51 & 2.52 & 1.93& 1.33 & 1.41 & 1.47 & 2.62 & 2.11 & 1.35 \\
%     POCO~\cite{boulch2022poco} & 1.77 & 2.10 & 2.68 & 1.40 & 1.54 & 2.93 & 1.78 & 1.50 & 1.39 & 1.46 & 2.55 & 1.83 & 1.40 \\
%     \midrule
%     % Ours ($N_{\text{Train}}$=$N_{\text{Test}}$=3k) & \textbf{1.02} & 1.36 & 1.78 & \textbf{1.00} & 1.07 & 1.91 & \textbf{1.47} & 0.88 & \textbf{0.87} & \textbf{1.03} & 1.91 & 1.36 & 0.80
% %   \\
%     % Ours ($N_{\text{Train}}$=$N_{\text{Test}}$=10k) & 1.03 &  \textbf{1.32} & \textbf{1.68} & 1.05 & \textbf{1.03} & \textbf{1.81} & 1.51 & \textbf{0.81} & 0.96 & 1.44 & \textbf{1.78} & \textbf{1.19} & \textbf{0.78}  \\
%     % Ours ($N_{\text{Train}}$=$N_{\text{Test}}$=10k) & 0.97 & 1.05 & 1.88 & \\
%     % Ours (w/ our decoder, $N_{\text{Train}}$=$N_{\text{Test}}$=3k) \\
%     ALTO & \textbf{1.11} & \textbf{1.42} & \textbf{1.71} & \textbf{1.18} & \textbf{1.24} & \textbf{1.86} & \textbf{1.43} & \textbf{0.87} & \textbf{1.10} & \textbf{1.16} & \textbf{1.87} &\textbf{1.50} & \textbf{0.84}\\
   
%   \bottomrule 
% % \hdashline
% % \end{tabular} \label{tab:vital}
% % \end{table*}
% % \begin{table*}
% % \centering
% %   \begin{tabular}{lccccccccc}
% %     \toprule
% \end{tabular}}\vspace{-2mm}
% \caption{\textbf{Quantitative results for model trained on ABC dataset and test results (Chamfer-$L_1$) on ABC test set, Famous, Things10k datasets are reported.} We strictly follow the experimental settings in~\cite{boulch2022poco}: $N_{\text{Train}}$=$N_{\text{Test}}$=10K and various point noise levels (`no-n.': no noise, `var-n': variable noise levels, `max-n': high noise level) and point density levels (`sparse': 5 scans, `dense': 30 scans) are used.}
% \label{tab:abc}
% \end{table*}


% As a result of Marching Cube, the vertices are usually placed in the middle of segments, which causes discretization effects~\cite{boulch2022poco}. To deal with this issue, we apply the refinement method from POCO~\cite{boulch2022poco}, which takes both the generated vertices and their floor to predict their occupancy values again. After that, we compare two values, mask out non-perfect vertices, take the average between the generated vertices and their floor, and repeat 10 times to improve the granularity.

% \begin{figure*}[t]
%   \centering
% %   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%   \includegraphics[width=\linewidth]{figures/skip_connection.JPG}

%   \caption{\textbf{draft figure here just for illustration.} expand on the point-grid alternating block and both point-wise and grid-wise skip connections between two consecutive layers}
%   \label{fig:onecol}
% \end{figure*}










\begin{figure*}[t]
%   \fbox{\rule{0pt}{6in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=\linewidth]{figures/synthetic_room/fig_synthetic_room_cropped.pdf}\vspace{-2mm}
\hfill\subcaptionbox{Ground Truth}[0.17\linewidth]
\hfill\subcaptionbox{Input Points}[0.14\linewidth]
\hfill\subcaptionbox{SPSR~\cite{kazhdan2013screened}}[0.22\linewidth]
\hfill\subcaptionbox{ConvONet~\cite{peng2020convolutional}}[0.15\linewidth]
\hfill\subcaptionbox{POCO~\cite{boulch2022poco}}[0.18\linewidth]
\hfill\subcaptionbox{\textbf{ALTO}}[0.13\linewidth]

\caption{\textbf{Qualitative comparison on scene-level reconstruction Synthetic Room Dataset.} Learning-based methods are trained and tested on 10K noisy points. ALTO can reconstruct the (top scene) double-deck table and (bottom scene) details in the chair.}
  \label{fig:syntheticroom}
%   \achuta{specify noise, e.g.g as pct of volume size noise - see previous paper.}
  % \achuta{(a) GT (b) Input .... (f) ours.}
\end{figure*}


\subsection{Results of Object-level Reconstruction}
\label{sec:object}

\textbf{Qualitative Object-level Comparisons:} Qualitative results of object-level reconstruction are provided in~\cref{fig:shapenet}. We observe that~\cite{peng2020convolutional} obtains a blurry reconstruction. Note that the width of the bookcase dividers are thicker and there are spurious blobs on the shelves. The SOTA baseline~\cite{boulch2022poco} is able to recover some detail, such as the wheel geometry in the car, but loses both side mirrors in the reconstruction. ALTO seems to have a higher fidelity reconstruction due to combining ideas from point and grid latents. 

\textbf{Quantative Object-level Comparisons:} ALTO's performance metrics at various point density levels are listed in~\cref{tab:shapenet}, for 3K, 1K and 300 input points. When point clouds are sparser, ALTO performs better than POCO on all four metrics. At high point density, ALTO outperforms POCO on three of four metrics. An ablation of just using the ALTO latent encoding and a traditional interpolating decoder~\cite{peng2020convolutional} is also conducted in the table. 
% In ~\cref{tab:abc} our method is compared quantitatively against Points2Surf~\cite{erler2020points2surf} and POCO~\cite{boulch2022poco} on both intra-dataset (train on ABC and test on ABC) and cross-dataset generalization settings (train on ABC and test on Famous and Things10k dataset). In tested conditions, including noise and noise-free conditions, ALTO is the top performing method.



% \begin{table}[t]
%     \label{tab:ubfc}
%     % \vskip 0.05in
%   \begin{center}
%   \resizebox{\linewidth}{!}{
%   \begin{tabular}{lccccccc} 
%     \toprule
  
%     Method & IoU $\uparrow$ & Chamfer-$L_1 \downarrow$ & NC$\uparrow$ & F-score$\uparrow$  \\
%     \midrule
% %   3D-CNN augmented & \textbf{3.32} & \textbf{4.01} &  \textbf{0.50} & \textbf{3.01}\\
% %   3D-CNN baseline & 3.53 & 4.24 &0.43 & 2.75\\
%   ONet~\cite{mescheder2019occupancy} & \\
%   SPSR~\cite{kazhdan2013screened} &  \\
%   SPSR trimmed~\cite{kazhdan2013screened} &  \\
%   ConvONet~\cite{peng2020convolutional} & \\
%   DP-ConvONet~\cite{lionar2021dynamic} & \\
%   POCO~\cite{boulch2022poco} & \\
%   \midrule
%   Ours & \\
%     \bottomrule
%   \end{tabular}}
%  \end{center}
%   \caption{\textbf{Performance on ShapeNet Dataset (partial input).} Boldface font represents the preferred results.}
% \end{table}

% \begin{table}[t]
%     \label{tab:shapenetsparse}
%     % \vskip 0.05in
%   \begin{center}
%   \resizebox{\linewidth}{!}{
%   \begin{tabular}{lccccccc} 
%     \toprule
  
%     Method & IoU $\uparrow$ & Chamfer-$L_1 \downarrow$ & NC$\uparrow$ & F-score$\uparrow$  \\
%     \midrule
%   ConvONet~\cite{peng2020convolutional} &  0.821 & 0.59 & 0.907 & 0.883
% \\
%   POCO~\cite{boulch2022poco} & 0.808 & 0.61 & 0.892 & 0.869
%  \\
%   \midrule
%   Ours &  0.842 & 0.52 & 0.908 & 0.903 \\
%   Ours (w/ our decoder) & \textbf{0.863} & \textbf{0.47} & \textbf{0.922} & \textbf{0.924} \\
%     \bottomrule
%   \end{tabular}}
%  \end{center}
%   \caption{\textbf{Performance on ShapeNet Dataset (sparser input).} Boldface font represents the preferred results.}
% \end{table}





% %%%%%%%%%%%%%%%%%%%%%%% vertical version %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newlength{\imagewidth}
% \begin{figure*}
% \def\arraystretch{0}% remove \arraystretch\dp\strutbox from row gap
% \setlength{\imagewidth}{\dimexpr \textwidth - 4\tabcolsep}% each gap takes 2\tabcolsep
% \divide \imagewidth by 5
% \hspace*{\dimexpr -\baselineskip - 2\tabcolsep}% move first column into margin

% \begin{tabular}{@{}cc@{}}
%   \raisebox{0.5\imagewidth}{\rotatebox[origin=c]{90}%
%     {\strut Input}} &
%   %\includegraphics[width=\imagewidth]{example-image-1x1} &
%   %\includegraphics[width=0.5\imagewidth]{example-image-1x1} &
%   %\includegraphics[width=0.5\imagewidth]{example-image-1x1} &
%   \includegraphics[width=0.9\linewidth]{figures/synthetic_room/synthetic_room_input.pdf} \\[0.2\tabcolsep]% adds gap between rows
  
%   \raisebox{0.5\imagewidth}{\rotatebox[origin=c]{90}%
%     {\strut SPSR~\cite{kazhdan2013screened}}} &
%   %\includegraphics[width=\imagewidth]{example-image-1x1} &
%   %\includegraphics[width=\imagewidth]{example-image-1x1} &
%   %\includegraphics[width=\imagewidth]{example-image-1x1} &
%   \includegraphics[width=0.93\linewidth]{figures/synthetic_room/synthetic_room_spsr.pdf} \\[0.2\tabcolsep]
  
%   \raisebox{0.5\imagewidth}{\rotatebox[origin=c]{90}%
%     {\strut ConvONet~\cite{peng2020convolutional}}} &
%   \includegraphics[width=0.93\linewidth]{figures/synthetic_room/synthetic_room_convonet.pdf} \\[0.25\tabcolsep]

%   \raisebox{0.5\imagewidth}{\rotatebox[origin=c]{90}%
%     {\strut POCO~\cite{boulch2022poco}}} &
%   \includegraphics[width=0.93\linewidth]{figures/synthetic_room/synthetic_room_poco.pdf} \\[0.2\tabcolsep]

%   \raisebox{0.5\imagewidth}{\rotatebox[origin=c]{90}%
%     {\strut Ours}} &
%   \includegraphics[width=0.93\linewidth]{figures/synthetic_room/synthetic_room_ours.pdf} \\[0.2\tabcolsep]

%   \raisebox{0.5\imagewidth}{\rotatebox[origin=c]{90}%
%     {\strut Ground Truth}} &
%   \includegraphics[width=0.93\linewidth]{figures/synthetic_room/synthetic_room_gt.pdf} %\\
%   %[0\tabcolsep]
  
%     %\setcounter{imagecolumn}{0} &% \stepcounter{imagerow} will also work
%     %Column \arabic{imagecolumn} &
%     %Column \arabic{imagecolumn} &
%     %Column \arabic{imagecolumn}
% \end{tabular}
% \caption{\textbf{Synthetic Room.} The methods train and test on 10k noisy points. \achuta{suggest tranpose this figure. yes it will be smaller, but it is currently taking up too much space IMHO.}\shijie{will do!}}
% \label{fig:room}
% \end{figure*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[t]

   
    % \vskip 0.05in
  \begin{center}
  \resizebox{\linewidth}{!}{
  \begin{tabular}{lccccccc} 
    \toprule
  
    Method & IoU $\uparrow$ & Chamfer-$L_1 \downarrow$ & NC$\uparrow$ & F-score$\uparrow$  \\
    \midrule
%   3D-CNN augmented & \textbf{3.32} & \textbf{4.01} &  \textbf{0.50} & \textbf{3.01}\\
%   3D-CNN baseline & 3.53 & 4.24 &0.43 & 2.75\\
   ONet~\cite{mescheder2019occupancy} & 0.475 &2.03& 0.783 & 0.541\\
  SPSR~\cite{kazhdan2013screened} & - & 2.23 & 0.866 & 0.810 \\
  SPSR trimmed~\cite{kazhdan2013screened} & - & 0.69 & 0.890 & 0.892 \\
  ConvONet~\cite{peng2020convolutional} & 0.849 & 0.42 & 0.915 & 0.964  \\
  DP-ConvONet~\cite{lionar2021dynamic} & 0.800 & 0.42 & 0.912 & 0.960  \\
  POCO~\cite{boulch2022poco} & 0.884 & 0.36 & 0.919 & 0.980
 \\
  \midrule
%   Ours ($ 3\times128^2$) &  0.834 & 0.43 & 0.906 & 0.960

% \\
%   Ours ($64^3$) &  0.903 & 0.36 & 0.920 & 0.978 \\
%%% 4heads hidden 128
ALTO & \textbf{0.914} & \textbf{0.35} & \textbf{0.921} & \textbf{0.981}\\
%%% 1head hidden 32 (1105 poco_mc)
%Ours (w/ our decoder, $64^3$) & \textbf{0.912} & \textbf{0.35} & \textbf{0.921} & \textbf{0.981}\\

    \bottomrule
  \end{tabular}}\vspace{-3mm}
 \end{center}
  \caption{\textbf{Synthetic Room Dataset.} Input points 10K with noise added. Boldface font represents the preferred results.}
   \label{tab:room}
\end{table}


\begin{table}[t]
    % \vskip 0.05in
  \begin{center}
  \resizebox{0.85\linewidth}{!}{
  \begin{tabular}{lccccccc} 
    \toprule
  
    Method & IoU $\uparrow$ & Chamfer-$L_1 \downarrow$ & NC$\uparrow$ & F-score$\uparrow$  \\
    \midrule
  ConvONet~\cite{peng2020convolutional} & 0.818 & 0.46 & 0.906 & 0.943 \\
  POCO~\cite{boulch2022poco} & 0.801 & 0.57 & 0.904 & 0.812  \\
  \midrule
  ALTO & \textbf{0.882} & \textbf{0.39} & \textbf{0.911} & \textbf{0.969} \\
    \bottomrule
  \end{tabular}}\vspace{-3mm}
 \end{center}
      \caption{\textbf{Performance on Synthetic Room Dataset (sparser input point cloud with 3K input points).} Boldface font represents the preferred results.}
\label{tab:room_sparse}
\end{table}



\subsection{Scene-level Reconstruction}
\label{sec:scene}

\textbf{Qualitative Scene-level Comparisons:} ALTO achieves detailed qualitative results compared to baselines. ~\cref{fig:syntheticroom} depicts scene-level reconstruction on the Synthetic Room dataset introduced in~\cite{peng2020convolutional}. In the first row of~\cref{fig:syntheticroom} the baselines of ConvONet and POCO both have holes in the coffee table. In the second row of~\cref{fig:syntheticroom} the high-frequency deatil in the wooden slats of the chair is fully blurred out by ConvONet. The advantages of ALTO are even more apparent for fine detail, such as the thin lamp-posts shown in ~\cref{fig:teaser}. ALTO reduces the quantization effect due to the grid discretization in the grid form by by using iterative alternation between grid and point latents, encoding more fine-grained local features for conditional occupancy field generation.

\textbf{Quantitative Scene-level Comparisons:} ALTO scores higher on quantitative values for scene-level metrics, shown in~\cref{tab:room} and~\cref{tab:room_sparse}. In the sparse setting, for the baselines methods, we find that ConvONet~\cite{peng2020convolutional} is quantitatively superior to the SOTA of POCO~\cite{boulch2022poco} because oversmoothing tends to improve quantitative results on noisy point clouds. Nonetheless, ALTO performs better than both baselines because ALTO limits spurious noise without resorting to as much oversmoothing. 







\subsection{Real-world Scene Generalization}
\label{sec:real}

\begin{figure*}[t]
%   \fbox{\rule{0pt}{3in} \rule{0.9\linewidth}{0pt}}

  \includegraphics[width=\linewidth]{figures/F_scannet.pdf}\vspace{-3mm}
\hfill\subcaptionbox{Ground Truth}[0.17\linewidth][l]
\hfill\subcaptionbox{Input Points}[0.16\linewidth]
\hfill\subcaptionbox{SPSR~\cite{kazhdan2013screened}}[0.18\linewidth][l]
\hfill\subcaptionbox{ConvONet~\cite{peng2020convolutional}}[0.14\linewidth]
\hfill\subcaptionbox{POCO~\cite{boulch2022poco}}[0.19\linewidth]
\hfill\subcaptionbox{\textbf{ALTO}}[0.13\linewidth]

  \caption{\textbf{Cross-dataset evaluation of ALTO and baselines by training on Synthetic Rooms~\cite{peng2020convolutional} and testing on real-world ScanNet-v2~\cite{Dai2017CVPR}}. Note the large conference-room table is missing in ConvONet~\cite{peng2020convolutional} (purple inset). The ladder (yellow inset) is a high-frequency surface and we believe our method is qualitatively closest. Please zoom in if browsing with PDF.} 
  \label{fig:scannet}
\end{figure*}

\begin{table}[t]
    % \vskip 0.05in
  \begin{center}
  \resizebox{\linewidth}{!}{
  \begin{tabular}{lccccccc} 
    \toprule
   \multirow{1}{*}{} & \multicolumn{2}{c}{\centering $N_{\text{Train}}$=10K, $N_{\text{Test}}$=3K} & \multicolumn{2}{c}{\centering $N_{\text{Train}}$=$N_{\text{Test}}$=3K} & \\
    \cmidrule(l){2-3} \cmidrule(l){4-5} 
    Method &  Chamfer-$L_1 \downarrow$  & F-score$\uparrow$& Chamfer-$L_1 \downarrow$  & F-score$\uparrow$ \\
    \midrule
%   ONet~\cite{mescheder2019occupancy} & 0.398 & 0.390\\
%   SPSR~\cite{kazhdan2013screened} & 0.293 & 0.731 \\
%   SPSR-trimmed~\cite{kazhdan2013screened} & 0.086 & 0.847 \\
  ConvONet~\cite{peng2020convolutional} & 1.01 & 0.719 &1.16 & 0.669\\
  POCO~\cite{boulch2022poco} & 0.93 & 0.737 & 1.15 & 0.667 \\ % 0.798\\
  \midrule
%   Ours & 0.95 & 0.745 & 0.98 & 0.827\\
  ALTO     & \textbf{0.87} & \textbf{0.746} & \textbf{0.92} & \textbf{0.726}\\
    \bottomrule
  \end{tabular}}
 \end{center}\vspace{-3mm}
  \caption{\textbf{ScanNet-v2.} We test the generalization capability of all the methods on real-world scans ScanNet using models trained on both the same input points of synthetic dataset as test set ($N_{\text{Train}}$=$N_{\text{Test}}$=3K) and different point density level ($N_{\text{Train}}$=10K, $N_{\text{Test}}$=3K). Boldface font represents the preferred results.   }
   \label{tab:scannet}
\end{table}

A final experiment in the main paper is to assess the performance of our model in real-world scans from ScanNet-v2~\cite{Dai2017CVPR}. All models are trained on Synthetic Rooms and tested on ScanNet-v2 to demonstrate generalization capability of our method along with baselines. We demonstrate the qualitative results of the setting where models trained
on both the same input points of synthetic dataset as ScanNet test set
($N_{\text{Train}}$=$N_{\text{Test}}$=3K) in~\cref{fig:scannet}. Our method is qualitatively superior to SPSR~\cite{kazhdan2013screened}, ConvONet~\cite{peng2020convolutional}, and POCO~\cite{boulch2022poco}. As in the Synthetic Rooms dataset, we observe that ConvONet oversmooths surfaces (sometimes causing entire objects to disappear, like the conference table in the purple inset of~\cref{fig:scannet}). In contrast, POCO retains some detail but is noisier. The quantitative results in~\cref{tab:scannet} are consistent with qualitative results. 
The cross point density test results ($N_{\text{Train}}$=10k, $N_{\text{Test}}$=3k) also demonstrates the superiority of our method on generalization when there are abundant input points in synthetic dataset used for training and low point density in real-world inference.

\begin{table}[t]
   
    % \vskip 0.05in
  \begin{center}
  \resizebox{0.8\linewidth}{!}{
  \begin{tabular}{lccccccc} 
    \toprule
  
    Method & $\#$ Parameters &  Inference time (s) \\
    \midrule
    % ConvONet ($3 \times 128^2$) & 7,812,705 & 1.80 & 0.97\\
    ConvONet~\cite{peng2020convolutional} & 4,166,657 & 1.6 \\ 
    POCO~\cite{boulch2022poco} & 12,790,454 & 36.1\\
    % \midrule
    % Ours ($3 \times 128^2$) & 2,713,889 & 1.74 & 4.86\\
    % Ours  ($64 ^3$) & 4,778,433 & 2.70 &4.48 \\
    % Ours (w/ our decoder, $3 \times 128^2$) & 2,763,073 & 3.00  & 6.93\\
    ALTO & 4,787,905&  3.6 \\
    \bottomrule
  \end{tabular}}
 \end{center}
  \caption{\textbf{Runtime comparison.} We report the number of parameters and inference time corresponding to~\cref{fig:scannet}. ALTO is much faster than POCO and recovers more detail~\cite{boulch2022poco}. ALTO is also only slightly slower than fast methods that are not as spatially expressive~\cite{peng2020convolutional}.}
   \label{tab:runtime}
\end{table}
% results on ScanNet-v2 and Matterport3D  

% \begin{table}[t]
%     \label{tab:ubfc}
%     % \vskip 0.05in
%   \begin{center}
%   %\resizebox{\linewidth}{!}{
%   \begin{tabular}{lccccccc} 
%     \toprule
  
%     Method &  Chamfer-$L_1 \downarrow$  & F-score$\uparrow$  \\
%     \midrule
%   ONet~\cite{mescheder2019occupancy} & 0.398 & 0.390\\
%   SPSR~\cite{kazhdan2013screened} & 0.293 & 0.731 \\
%   SPSR-trimmed~\cite{kazhdan2013screened} & 0.086 & 0.847 \\
%   ConvONet~\cite{peng2020convolutional} & 0.094\\
%   POCO~\cite{boulch2022poco} & \\
%   \midrule
%   Ours & \\
%     \bottomrule
%   \end{tabular}
%  \end{center}
%   \caption{\textbf{Performance on ScanNet-v2.} Boldface font represents the preferred results.}
% \end{table}



% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%   \caption{a plot showing various densities}
%   \label{fig:onecol}
% \end{figure}









==> point-grid-alternating-cvpr2023 (Copy) (1)/shortcuts.tex <==
% shortcuts for bold characters (vectors, matrices)
\newcommand{\ba}{\mathbf{a}}\newcommand{\bA}{\mathbf{A}}
\newcommand{\bb}{\mathbf{b}}\newcommand{\bB}{\mathbf{B}}
\newcommand{\bc}{\mathbf{c}}\newcommand{\bC}{\mathbf{C}}
\newcommand{\bd}{\mathbf{d}}\newcommand{\bD}{\mathbf{D}}
\newcommand{\be}{\mathbf{e}}\newcommand{\bE}{\mathbf{E}}
\newcommand{\bff}{\mathbf{f}}\newcommand{\bF}{\mathbf{F}} %\bf already taken
\newcommand{\bg}{\mathbf{g}}\newcommand{\bG}{\mathbf{G}}
\newcommand{\bh}{\mathbf{h}}\newcommand{\bH}{\mathbf{H}}
\newcommand{\bi}{\mathbf{i}}\newcommand{\bI}{\mathbf{I}}
\newcommand{\bj}{\mathbf{j}}\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bk}{\mathbf{k}}\newcommand{\bK}{\mathbf{K}}
\newcommand{\bl}{\mathbf{l}}\newcommand{\bL}{\mathbf{L}}
\newcommand{\bm}{\mathbf{m}}\newcommand{\bM}{\mathbf{M}}
\newcommand{\bn}{\mathbf{n}}\newcommand{\bN}{\mathbf{N}}
\newcommand{\bo}{\mathbf{o}}\newcommand{\bO}{\mathbf{O}}
\newcommand{\bp}{\mathbf{p}}\newcommand{\bP}{\mathbf{P}}
\newcommand{\bq}{\mathbf{q}}\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\br}{\mathbf{r}}\newcommand{\bR}{\mathbf{R}}
\newcommand{\bs}{\mathbf{s}}\newcommand{\bS}{\mathbf{S}}
\newcommand{\bt}{\mathbf{t}}\newcommand{\bT}{\mathbf{T}}
\newcommand{\bu}{\mathbf{u}}\newcommand{\bU}{\mathbf{U}}
\newcommand{\bv}{\mathbf{v}}\newcommand{\bV}{\mathbf{V}}
\newcommand{\bw}{\mathbf{w}}\newcommand{\bW}{\mathbf{W}}
\newcommand{\bx}{\mathbf{x}}\newcommand{\bX}{\mathbf{X}}
\newcommand{\by}{\mathbf{y}}\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bz}{\mathbf{z}}\newcommand{\bZ}{\mathbf{Z}}

% shortcuts for bold greek characters (vectors, matrices)
\newcommand{\balpha}{\boldsymbol{\alpha}}\newcommand{\bAlpha}{\boldsymbol{\Alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}\newcommand{\bBeta}{\boldsymbol{\Beta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\bdelta}{\boldsymbol{\delta}}\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}\newcommand{\bEpsilon}{\boldsymbol{\Epsilon}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}\newcommand{\bZeta}{\boldsymbol{\Zeta}}
\newcommand{\beeta}{\boldsymbol{\eta}}\newcommand{\bEta}{\boldsymbol{\Eta}} % \beta already taken
\newcommand{\btheta}{\boldsymbol{\theta}}\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\biota}{\boldsymbol{\iota}}\newcommand{\bIota}{\boldsymbol{\Iota}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}\newcommand{\bKappa}{\boldsymbol{\Kappa}}
\newcommand{\blambda}{\boldsymbol{\lambda}}\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bmu}{\boldsymbol{\mu}}\newcommand{\bMu}{\boldsymbol{\Mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}\newcommand{\bNu}{\boldsymbol{\Nu}}
\newcommand{\bxi}{\boldsymbol{\xi}}\newcommand{\bXi}{\boldsymbol{\Xi}}
\newcommand{\bomikron}{\boldsymbol{\omikron}}\newcommand{\bOmikron}{\boldsymbol{\Omikron}}
\newcommand{\bpi}{\boldsymbol{\pi}}\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\brho}{\boldsymbol{\rho}}\newcommand{\bRho}{\boldsymbol{\Rho}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\btau}{\boldsymbol{\tau}}\newcommand{\bTau}{\boldsymbol{\Tau}}
\newcommand{\bypsilon}{\boldsymbol{\ypsilon}}\newcommand{\bYpsilon}{\boldsymbol{\Ypsilon}}
\newcommand{\bphi}{\boldsymbol{\phi}}\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bchi}{\boldsymbol{\chi}}\newcommand{\bChi}{\boldsymbol{\Chi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bomega}{\boldsymbol{\omega}}\newcommand{\bOmega}{\boldsymbol{\Omega}}

% shortcuts for blackboard bold characters (eg, number sets)
\newcommand{\nA}{\mathbb{A}}
\newcommand{\nB}{\mathbb{B}}
\newcommand{\nC}{\mathbb{C}}
\newcommand{\nD}{\mathbb{D}}
\newcommand{\nE}{\mathbb{E}}
\newcommand{\nF}{\mathbb{F}}
\newcommand{\nG}{\mathbb{G}}
\newcommand{\nH}{\mathbb{H}}
\newcommand{\nI}{\mathbb{I}}
\newcommand{\nJ}{\mathbb{J}}
\newcommand{\nK}{\mathbb{K}}
\newcommand{\nL}{\mathbb{L}}
\newcommand{\nM}{\mathbb{M}}
\newcommand{\nN}{\mathbb{N}}
\newcommand{\nO}{\mathbb{O}}
\newcommand{\nP}{\mathbb{P}}
\newcommand{\nQ}{\mathbb{Q}}
\newcommand{\nR}{\mathbb{R}}
\newcommand{\nS}{\mathbb{S}}
\newcommand{\nT}{\mathbb{T}}
\newcommand{\nU}{\mathbb{U}}
\newcommand{\nV}{\mathbb{V}}
\newcommand{\nW}{\mathbb{W}}
\newcommand{\nX}{\mathbb{X}}
\newcommand{\nY}{\mathbb{Y}}
\newcommand{\nZ}{\mathbb{Z}}

% shortcuts for calligraphic characters (sets, index sets, ...)
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\co}{\mathcal{o}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

% references to figures, sections, algorithms, equations, tables
% \newcommand{\figref}[1]{Fig.~\ref{#1}}
% \newcommand{\secref}[1]{Section~\ref{#1}}
% \newcommand{\algref}[1]{Algorithm~\ref{#1}}
% \newcommand{\eqnref}[1]{Eq.~\eqref{#1}}
% \newcommand{\tabref}[1]{Table~\ref{#1}}

% argmin / argmax operators
\DeclareMathOperator*{\argmax}{argmax~}
\DeclareMathOperator*{\argmin}{argmin~}
\DeclareMathOperator{\EX}{\mathbb{E}}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\relu}{relu}

% mathcal / mathbf shortcuts
\def\mc{\mathcal}
\def\mb{\mathbf}

% nice transpose operator
\newcommand{\T}{^{\raisemath{-1pt}{\mathsf{T}}}}

% statistical dependency symbol (_||_)
\newcommand{\Perp}{\perp\!\!\! \perp}

% shortcuts for: \eg, \ie, \cf, \etc, \vs, \wrt, \dof, \etal, \iid
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{e.g\onedot} \def\Eg{E.g\onedot}
\def\ie{i.e\onedot} \def\Ie{I.e\onedot}
\def\cf{cf\onedot} \def\Cf{Cf\onedot}
\def\etc{etc\onedot}
\def\vs{vs\onedot}
\def\wrt{wrt\onedot}
\def\dof{d.o.f\onedot}
\def\etal{et~al\onedot}
\def\iid{i.i.d\onedot}
\makeatother

% nice url font and color
\renewcommand\UrlFont{\color{blue}\rmfamily}

% rotation
\newcommand*\rot{\rotatebox{90}}

% boldparagraph for unnumbered sections
\newcommand{\boldparagraph}[1]{\vspace{0.2cm}\noindent{\bf #1:} }

\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\tabref}[1]{Tab.~\ref{#1}}
\newcommand{\secref}[1]{Sec.~\ref{#1}}

% custom color definitions
\definecolor{darkred}{rgb}{0.7,0.2,0.1}
\definecolor{darkgreen}{rgb}{0,0.7,0}
\definecolor{orange}{RGB}{255,127,0}
\definecolor{ourpurple}{RGB}{127,127,204}
\definecolor{palgreen}{RGB}{51,179,179}
\definecolor{magenta}{RGB}{199,21,133}

% commands for comments
\newcommand{\red}[1]{\noindent{\color{red}{#1}}}
\newcommand{\desp}[1]{ \noindent {\color{cyan} {\bf Despoina:} {#1}} }

